SV4D 2.0: Enhancing Spatio-Temporal Consistency in Multi-View Video Diffusion for High-Quality 4D Generation

We present Stable Video 4D 2.0 (SV4D 2.0), a multi-view video diffusion model for dynamic 3D asset generation. Compared to its predecessor SV4D, SV4D 2.0 is more robust to occlusions and large motion, generalizes better to real-world videos, and produces higher-quality outputs in terms of detail sharpness and spatio-temporal consistency. We achieve this by introducing key improvements in multiple aspects: 1) network architecture: eliminating the dependency of reference multi-views and designing blending mechanism for 3D and frame attention, 2) data: enhancing quality and quantity of training data, 3) training strategy: adopting progressive 3D-4D training for better generalization, and 4) 4D optimization: handling 3D inconsistency and large motion via 2-stage refinement and progressive frame sampling. Extensive experiments demonstrate significant performance gain by SV4D 2.0 both visually and quantitatively, achieving better detail (-14\% LPIPS) and 4D consistency (-44\% FV4D) in novel-view video synthesis and 4D optimization (-12\% LPIPS and -24\% FV4D) compared to SV4D. Project page: https://sv4d20.github.io.

==> sec/0_abstract.tex <==
\begin{abstract}
%
We present Stable Video 4D 2.0 (SV4D 2.0), a multi-view video diffusion model for dynamic 3D asset generation. Compared to its predecessor SV4D~\cite{xie2024sv4d}, SV4D 2.0 is more robust to occlusions and large motion, generalizes better to real-world videos, and produces higher-quality outputs in terms of detail sharpness and spatio-temporal consistency. We achieve this by introducing key improvements in multiple aspects: 1) network architecture: eliminating the dependency of reference multi-views and designing blending mechanism for 3D and frame attention, 2) data: enhancing quality and quantity of training data, 3) training strategy: adopting progressive 3D-4D training for better generalization, and 4) 4D optimization: handling 3D inconsistency and large motion via 2-stage refinement and progressive frame sampling. Extensive experiments demonstrate significant performance gain by SV4D 2.0 both visually and quantitatively, achieving better detail (-14\% LPIPS) and 4D consistency (-44\% FV4D) in novel-view video synthesis and 4D optimization (-12\% LPIPS and -24\% FV4D) compared to SV4D. 
%
\end{abstract}


% SV4D 2.0 
% Datasets
% - Pretrain on 3D datasets
% - Improve ObjaverseDy data
% - Increase the data scale/quality with ObjaverseXL (27K -> ~160K) (in progress)
% - Incorporate real-world video data (to-do)
% Model architecture
% - Optional mv condition
% - Use camera embedding in camera_attention
% - Relative elevation 
% 3D attention: merge spatial and view axes
% Add 12-frame-4-view model

% Story:
% Get rid of the constraints of mv condition
% Improving dataset in both scale and quality


==> tables/efficiency.tex <==
\definecolor{best}{rgb}{0.996, 0.769, 0.3098}
\newcommand{\C}{\cellcolor{best}}

\definecolor{second}{rgb}{1, 0.969, 0.733}
\newcommand{\CC}{\cellcolor{second}}

\begin{table}[!h]
%\caption{
%\textbf{Efficiency Analysis.} 
%}
\vspace{-.75em}
\label{tab:efficiency}
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{0.81\linewidth}{!}{
\begin{tabular}{ l c c c c c c c c c}
% \toprule 
  & Ours & w/o 3DAtt. & SV4D & Cons.[19] & STAG4D & DG4D[39] & Diffusion$^2$  & 4Diff[70] & L4GM\\
 \midrule
 Time$\downarrow$ & 22min  & 22min & 23min & 2 Hr & 1Hr & 12min & 20min & 8Hr & 3s\\
 % Mem$\downarrow$ & 30G & 26G & 26G & 24G & 15G & 70G & 320G (8 GPUs) & 50G & 16G \\
 Mem$\downarrow$ & 30G & 26G & 26G & 24G & 15G & 70G & 320G & 50G & 16G \\
% \bottomrule
\end{tabular}
}
\end{table}
